Sparse Voxels Rasterization: Real-time High-fidelity Radiance Field Rendering

We propose an efficient radiance field rendering algorithm that incorporates a rasterization process on adaptive sparse voxels without neural networks or 3D Gaussians. There are two key contributions coupled with the proposed system. The first is to adaptively and explicitly allocate sparse voxels to different levels of detail within scenes, faithfully reproducing scene details with $65536^3$ grid resolution while achieving high rendering frame rates. Second, we customize a rasterizer for efficient adaptive sparse voxels rendering. We render voxels in the correct depth order by using ray direction-dependent Morton ordering, which avoids the well-known popping artifact found in Gaussian splatting. Our method improves the previous neural-free voxel model by over 4db PSNR and more than 10x FPS speedup, achieving state-of-the-art comparable novel-view synthesis results. Additionally, our voxel representation is seamlessly compatible with grid-based 3D processing techniques such as Volume Fusion, Voxel Pooling, and Marching Cubes, enabling a wide range of future extensions and applications.

==> fig/demo_future.tex <==
\begin{figure}
    \centering
    % \begin{tabular}{@{}l@{}}
    % TSDF fusion without training ($\sim$ 3 sec)\\
    % \includegraphics[width=\linewidth]{img/demo_tsdf_fusion_row1.pdf} \\
    % Refining 1K iterations ($\sim$ 10 secs)\\
    % \includegraphics[width=\linewidth]{img/demo_tsdf_fusion_row2.pdf}
    % \end{tabular}
    \includegraphics[width=.95\linewidth]{img/demo_future.pdf}
    \vspace{-1em}
    \caption{
    {\bf Demonstration of applying Visual-Hull carving.}
    We show the potential of integrating some other useful grid-based algorithms into our sparse voxels representations.
    Given images with foreground masks, we can instantly mask carve a sparse grid with constant density and base color in less than 100ms, whose appearance and geometry can then be refined by optimizing the rendering losses.
    % In \cref{ssec:exp_mesh_extract}, we use TSDF Fusion and Marching Cubes to extract mesh from the optimized grid layout and density field.
    % We can also fuse from sensor depths to initialize our sparse voxels.
    % As we still can not render SDF, we naively apply linear transform to map the fused TSDF to density to showcase the results in this figure.
    }
    \label{fig:exp_tsdf_fusion}
\end{figure}

==> fig/exp_tsdf_fusion.tex <==
\begin{figure}
    \centering
    \begin{tabular}{@{}l@{}}
    TSDF fusion without training ($\sim$ 3 sec)\\
    \includegraphics[width=\linewidth]{img/demo_tsdf_fusion_row1.pdf} \\
    Refining 1K iterations ($\sim$ 10 secs)\\
    \includegraphics[width=\linewidth]{img/demo_tsdf_fusion_row2.pdf}
    \end{tabular}
    \vspace{-1em}
    \caption{
    {\bf Demonstration of applying TSDF fusion.}
    We can also integrate TSDF fusion into our \ourshortname if the sensor depth is provided. 
    In this indoor scene, we use voxel size in 2.5cm and truncated the signed distance to 3cm.
    The integrated \ourshortname with VolSDF~\cite{volsdf} enable us to start from a good and smooth initial surface as shown in the rendered depth and normal maps.
    Refining for additional 1K iterations achieve reasonable novel-view synthesis quality.
    }
    \label{fig:exp_tsdf_fusion}
\end{figure}

==> fig/exp_visual_hull.tex <==
\begin{figure}
    \centering
    \begin{tabular}{@{}l@{}}
    Input frames\\
    \includegraphics[width=\linewidth]{img/demo_visual_hull_gt.pdf} \\
    Visual hull without training (\textless 0.1 sec)\\
    \includegraphics[width=\linewidth]{img/demo_visual_hull_iter0.pdf} \\
    Refining 1K iterations (\textless 10 secs)\\
    \includegraphics[width=\linewidth]{img/demo_visual_hull_iter1k.pdf}
    \end{tabular}
    \vspace{-1em}
    \caption{
    {\bf Demonstration of applying visual hull.}
    In this example, we take about 60 frames with object masks as input.
    We show the novel-view synthesis results by incorporating visual hull into our \ourshortname.
    This can largely accelerate the convergence of object reconstruction given the object masks.
    }
    \label{fig:exp_visual_hull}
\end{figure}

==> fig/voxel_fields.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{img/voxel_fields.pdf}
    \caption{
        {\bf Voxel fields.}
        {\bf (Left)} In constant voxel field, the modal of interest is directly attached to the voxel and are constant everywhere inside the voxel.
        {\bf (Right)} For tri-linear voxel field, the modal to optimize is associated to voxel corner positions and tri-linearly vary within the voxel.
        We store the pointers to a grid points feature pool $\gridmod$ so the parameters can be shared between adjacent voxels.
        Refer to \cref{ssec:sparse_grid_layout} for details.
    }
    \label{fig:voxel_field}
\end{figure}

==> sec/1_intro_old.tex <==
\section{Introduction}
\label{sec:intro}

% [Cheng]: Starting from a higher level description might be better. If I have time....

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Previous writing is located at /sec/legacy/1_intro.tex % 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% In recent years, differentiable volume rendering has made significant strides in 3D scene reconstruction and novel-view synthesis tasks. Neural Radiance Fields (NeRF)~\cite{nerf} laid the foundation for this progress by optimizing a volumetric function, parameterized by multi-layer perceptrons (MLPs) to encode both geometry and appearance through differential rendering. 
% Despite its high-quality novel-view synthesis results, this pioneering study encounters inefficiency problems, primarily due to the need for evaluating large MLPs for hundreds of sampled points along each pixel ray during volume rendering, \aka ray casting. 
% This leads to a computationally expensive and slow rendering process.
% Subsequent studies focus on rendering speed acceleration by decomposing large MLPs into grid-based representations with shallow MLPs~\cite{dvgo,tensorf,instant-ngp}. 
% Depending on types of grid representations, grid-based NeRFs are categorized as dense grids~\cite{dvgo}, sparse grids~\cite{plenoxels}, factorized grids~\cite{tensorf}, tri-planes~\cite{eg3d}, and hash grids~\cite{instant-ngp}.
% These grid-based NeRFs have demonstrated the ability to achieve rendering quality comparable to fully MLP-based NeRFs while significantly reducing training time. Moreover, they enable real-time rendering, achieving frame rates of several frames per second (FPS), thus making them more suitable for practical applications.
% These grid-based NeRFs enable real-time rendering, achieving frame rates of several frames per second (FPS), thus making them more suitable for practical applications.
% While grid representations provide high-quality novel-view synthesis with faster rendering times, NeRF-based methods still rely on exhaustive ray casting, which involves sampling hundreds of points along each pixel ray in volume rendering. This can create computational bottlenecks.
% [Cheng]: The above description is not precise. 3DGS still visits hundreds of Gaussians for each ray. Just that (1) checking each Gaussians is very quick and (2) some computation of each primitive (mainly the SH to rgb) can be shared by all the pixels. Let make it more brief here and detailed discussion later in related work.

Recently, Kerbl~\etal~\cite{3dgs} introduced 3D Gaussian Splatting (3DGS), that leverages rasterization of a splatting algorithm~\cite{ewa} over an anisotropic 3D Gaussian representation to model 3D scenes from multi-views. This approach achieves real-time rendering speeds—exceeding 100 FPS—even for unbounded scenes.

However, 3DGS still has two major limitations.
First, the sorting of Gaussian centers does not guarantee proper depth ordering, which results in a popping artifact~\cite{stopthepop}.
% Second, the 3D volume is ill-defined as their splatting algorithm map 3D Gaussians to 2D Gaussians for pixels to query, without attributing the contribution back to specific 3D positions.
Second, the 3D volume is ill-defined when a 3D point is covered by multiple 3D Gaussians, as their rendering algorithm assumes the Gaussians always have a front-back order.
Due to this ambiguous volume representation, 3DGS-based surface reconstruction methods need to adopt  more complex post-processing algorithms~\cite{sugar} or rely on another grid-based representation to perform TSDF-Fusion and Marching Cubes for mesh extraction~\cite{2dgs}.

% the nature of 3D Gaussian distributions, which are known for their long-tail shape, complicates defining clear surface boundaries.
% Due to this ambiguous volume representation, 3DGS-based surface reconstruction methods~\cite{2dgs,sugar} typically require post-processing to convert Gaussian distributions into volumetric grid representations—a step generally unnecessary in NeRF-based approaches~\cite{neuralpbir,neuralangelo}.
% ......
% Second, 3DGS is not be directly compatible with many useful 3D processing algorithms.
% For instances, in surface reconstruction task, SuGaR~\cite{sugar} needed to invent a new mesh extraction algorithm.
% Instead of extracting meshes from Gaussians, 2DGS~\cite{2dgs} relies on another grid-based method for meshes from its rendered depths.
% However, 3DGS~\cite{3dgs} presents two main challenges.
% During the rasterization process, 3D Gaussians are sorted along pixel rays based on Gaussian centers rather than precise depth computation, resulting in multi-view inconsistencies and causing "popping" artifacts~\cite{stopthepop}.
% Additionally, the nature of 3D Gaussian distributions, which are known for their long-tail shape, complicates defining clear surface boundaries.
% Due to this ambiguous volume representation, 3DGS-based surface reconstruction methods~\cite{2dgs,sugar} typically require post-processing to convert Gaussian distributions into volumetric grid representations—a step generally unnecessary in NeRF-based approaches~\cite{neuralpbir,neuralangelo}.
% Despite this success, 3DGS has several limitations. In the rasterization process, the Z-depth of the mean is used to order 3D Gaussians which may lead to multi-view inconsistency, causing a so-called {\em popping artifact}~\cite{stopthepop}. 
% As a result of this ambiguous volumetric representation \charles{(the previous sentence doesn't make this point)}, state-of-the-art 3DGS-based mesh reconstruction methods~\cite{2dgs,sugar} need to design post-processing algorithms to get a volume grid, while NeRF-based methods have a meaningful volume for mesh extraction and maintain state-of-the-art quality~\cite{neuralpbir,neuralangelo}.

On the other hand, the volumetric representations of fully-MLP NeRFs~\cite{nerf,mip-nerf,mip-nerf360,neus,volsdf}, grid-based NeRFs~\cite{dvgo,tensorf,eg3d,neuralpbir,voxurf,neuralangelo}, and neural-free sparse voxels~\cite{plenoxels} do not suffer from the ordering issue and their volumes are well-defined.
However, the rendering speed of these methods are one to two orders of magnitude slower than 3DGS methods.

% Our motivation is to combine the strengths of GS-based and volumetric-based methods.
% Quick question -- what is the key advantage of SV vs GS? besides poping effect and natural integration with classic algorithms?
% I think these are the two main points. The well-defined volume (two paragraph above) is also a thing.
% sounds good
% Voxel gird is probably more directly compatible/integratable to many other thing/technique but I can't find all of them now. Future cool guys can show this.
Our motivation is to combine the efficiency strength of GS-based rendering approach into the volumetric-based scene representation.
In particularly, the neural-free sparse voxels, done by Plenoxels~\cite{plenoxels}, as it is a fully-explicit representation similar to 3DGS.
Both methods directly define the geometry and appearance of each voxel or Gaussian without relying on neural networks, making voxel computation as efficient as that for Gaussians.
The success of 3DGS can thus theoretically be replicated to a neural-free sparse voxel representation, while retaining all the benefits of a volumetric approach.

In our observation, the efficiency of 3DGS stems from its use of a rasterizer and the simple computation of its 3D primitives, while its high fidelity is achieved through adaptive control of primitive allocation to model different scene levels of detail.
Voxels are already as efficient to compute as Gaussians, so the remaining challenge is to extend uniform-sized sparse voxels to adaptive-sized sparse voxels and to implement a rasterizer suited for them.

In this work, we present \ourshortname, a novel framework that combines the efficiency of rasterization in 3DGS with the structured volumetric approach of grid-based representations.
\ourshortname leverages (1) multi-level sparse voxels to model 3D scenes and (2) implements a dynamic Morton order encoding that enables rasterization process from our adaptive-sized sparse voxel representation.
% Such a design can resolve the view-dependent artifacts and popping effects typically encountered in rasterization approaches like 3DGS~\cite{3dgs}. 
Our rendering is free from popping artifacts because the 3D space is partitioned into disjoint voxels, and our sorting ensures the correct rendering order.
Moreover, thanks to volumetric nature and neural-free representation of \ourshortname, our sparse voxel grid can be easily and seamlessly integrated with classical grid-based 3D processing algorithms, as demonstrated with the incorporated sparse-voxel TSDF Fusion and Marching Cubes.
% Our \ourshortname models 3D scenes as hierarchical sparse voxels, drawing on the strengths of both voxel grids and rasterization to achieve high performance. Based on this grid layout,
% Our \ourshortname models 3D scenes as sparse voxels in a grid layout, drawing on the strengths of both voxel grids and rasterization to achieve high performance. Specifically, we leverage an Octree layout for adaptive detail representation across different scene regions, while avoiding traditional Octree data structures such as parent-child pointers and overlapping voxels. Instead, 
% our approach relies on a custom multi-level Z-order encoding to maintain a consistent front-to-back rendering order, which mitigates the view-dependent artifacts and popping effects typically encountered in rasterization approaches like 3DGS~\cite{3dgs}. Our framework adheres to the volumetric rendering principles of grid-based NeRF~\cite{dvgo,plenoxels,instant-ngp}, producing visually accurate results at over 100 FPS for one-megapixel images. 
% The explicit and volumetric nature of \ourshortname enables directly using classic grid-based techniques for practical applications. For instance, sparse voxels in \ourshortname can model Signed Distance Functions (SDF) to support mesh extraction via marching cubes. Additionally, we incorporate gradient-free methods to leverage per-frame priors, such as visual hulls derived from object masks and TSDF fusion from sensor depth data. This capability allows for instant object reconstruction in under 0.1 seconds and facilitates smooth initial surface generation for complex indoor scenes, a feat not readily achievable with 3DGS alone.

% Through extensive experiments, we demonstrate that \ourshortname successfully combines the strengths of grid-based volumetric approach and the efficiency of 3DGS by using rasterization, offering a solution that balances rendering quality, computational efficiency, and versatility for enabling future pipelines to incorporate grid-based processing algorithm into our scene modeling approach.
We show that our method is training fast, rendering fast, and achieves novel-view synthesis quality comparable to the state-of-the-art.
We extract meshes by the integrated sparse-voxel TSDF-Fusion and sparse-voxel Marching Cubes from the trained sparse voxel grids.
Results on mesh reconstruction benchmarks show our good balance between surface accuracy and processing speed.


==> sec/legacy/1_intro.tex <==
\section{Introduction}
\label{sec:intro}

% \textcolor{blue}{jchoe$>$@Cheng. I will go over it again after having dinner.}
% \chengs{chengs$>$Thanks a lot! Please take your time :)}


%
% Discuss NeRF-family 
%
% Differentiable volume rendering for 3D scene reconstruction and novel-view synthesis has progressed rapidly in recent years.
% At the beginning, NeRF~\cite{nerf} achieves promising novel-view rendering quality by optimizing a MLP-parameterized volumetric function to reproduce the training views with differentiable rendering.
% One main drawback of NeRF is the inefficient rendering due to the computation of MLPs for hundreds of sample points per-pixel in the volume ray casting process.
% Subsequent works speedup rendering by incorporating grid-based representation into the scene functions, such as dense grid~\cite{dvgo}, sparse grid~\cite{plenoxels}, factorized grid~\cite{tensorf}, and hash grid~\cite{instant-ngp}, which are typically followed by a MLP for better scene smoothness.
% These grid-based methods achieve comparable quality than the fully-MLP NeRF while using much less training time, and attain dozen FPS.

In recent years, differentiable volume rendering has made significant strides in 3D scene reconstruction and novel-view synthesis tasks. Neural Radiance Fields (NeRF)~\cite{nerf} laid the foundation for this progress by introducing a method that optimizes a volumetric function parameterized by a multi-layer perceptron (MLP) to encode both geometry and appearance through differential rendering. Despite its high-quality novel-view synthesis, NeRF suffers from inefficiencies, primarily due to the need for evaluating a large MLP for hundreds of sampled points along each pixel ray during volume rendering. This leads to a computationally expensive and slow rendering process.

To overcome these limitations, subsequent works have focused on accelerating rendering through the integration of grid-based representations within the scene function. These include dense grids~\cite{dvgo}, sparse grids~\cite{plenoxels}, factorized grids~\cite{tensorf}, and hash grids~\cite{instant-ngp}, often augmented by a lightweight MLP to ensure smoothness in the scene representation. These grid-based methods have demonstrated the ability to achieve rendering quality comparable to fully MLP-based NeRFs while significantly reducing training time. Moreover, they enable real-time rendering, achieving frame rates of several frames per second (FPS), thus making them more suitable for practical applications.


%
% Discuss the strength of 3DGS
%
% Later, 3D Gaussians Splatting (3DGS)~\cite{3dgs} is proposed which uses a set of anisotropic 3D Gaussians as the scene function and achieve \textgreater 100 FPS even in unbounded scenes, which is an order magnitude faster than the grid-based NeRFs.
% One efficiency advantage of 3DGS comes from rasterization process as the rendering function instead of using volume ray casting employed by grid-based NeRF.
% We are motivated by the following properties about the scene representing due to the rasterization.
% The first is the flexibility about the data structure.
% Each Gaussian can adapt freely and explicitly to different level-of-details of the scene without limited by certain data structure like the n-d array or hash grid (will come back to this point later).
% Second is about the sparsity of the scene representation (it does not mean it use less parameters).
% Even the grid-based NeRF still need to maintain and query a dense occupancy grid to skip empty space for speedup, while 3DGS just need to iterate through the allocated Gaussians.

More recently, Kerbl~\etal~\cite{3dgs} propose 3D Gaussian Splatting (3DGS) which adopts a set of anisotropic 3D Gaussians as a scene function and achieve impressive rendering speed in excess of $100$ FPS even in unbounded scenes. Compared to NeRF~\cite{nerf}, the efficiency advantage in 3DGS comes from a rasterization stage that replaces the exhaustive volume ray casting employed by NeRF and subsequent works~\cite{nerf,dvgo,plenoxels,tensorf,instant-ngp}. 



%
% Discuss the weakness of 3DGS
%
% However, one biggest drawback of 3DGS comparing to NeRF is the lack of meaningful volumetric function.
% In NeRF, a volumetric function mapping a point in space to modal of interest is required in volume ray casting and explicitly trained.
% In 3DGS, such a function is ambiguous as the 3D Gaussians is approximately projected as 2D Gaussians lacking clear attribution to certain 3D region.
% In case of overlapping, the Gaussians are still treated as non-overlapping and the rendering order is also inconsistent across nearby view, which causes popping artifact~\cite{stopthepop}.
% In addition, the ill-defined volumetric function make it difficult to decide if a point is inside or outside the surface.
% As a result, GS-based mesh reconstruction methods~\cite{sugar,2dgs,gof} need to use rendered depths or a work around post-processing while NeRF-based methods have a meaningful volumetric function ready for marching cubes and still have the state-of-the-art quality~\cite{neuralpbir,neuralangelo}.

Despite this success, 3DGS has several limitations. 
%
%
% The 3DGS representation consists of a set of the 3D Gaussians whose location, shape, and appearance are defined by a mean, covariance matrix, and low-order spherical harmonics coefficients optimized so that their 2D projections closely match a set of training views. As such, it is difficult to define a clear decision boundary that defines a 3D surface. The Z-depth of the mean used to order these 2D projections may be multi-view inconsistent, causing a so-called {\em popping artifact}~\cite{stopthepop}.
In the rasterization process, the Z-depth of the mean is used to order 3D Gaussians and this can results in multi-view inconsistency, causing a so-called {\em popping artifact}~\cite{stopthepop}.
%
%
As a result of this ambiguous volumetric representation, state-of-the-art 3DGS-based mesh reconstruction methods~\cite{2dgs,gof} need to design post-processing algorithms to get a volume grid, while NeRF-based methods have a meaningful volume for mesh extraction and maintain state-of-the-art quality~\cite{neuralpbir,neuralangelo}.



%
% Our motivation
%

% \jchoe{Hey Cheng, It is highly difficult to follow the context below. I understand your intention but I hope we can further simplify the writing.}


We introduce \emph{\ourfullname~(\ourshortname)}, that combines the efficiency of the 3DGS framework with the well-defined surfaces of grid-based NeRF methods. Our \ourshortname describes 3D scenes as a set of sparse voxels like grid-based NeRF, and crucially, we leverage rasterization as our rendering function like 3DGS.
The key is the design of the voxel grid layout and the grid-specific rasterization algorithm.
We allocate voxels using an Octree layout so we can adapt the sparse voxels to different scene levels-of-detail, yet we do not maintain the Octree hierarchy or classical Octree data structure, \ie, no overlapping voxels with leaf nodes only, and no Octree parent and children pointers in our representation. 
In our rasterizer, the voxel rendering order is determined by sorting so we do not need Octree traversal.
We design a multi-level Z-order encoding to ensure a correct front-to-back rendering order that prevents the multi-view order inconsistent issue and the popping artifact of 3DGS.
Finally, the rasterization of each voxel fully respects the 3D volumetric rendering formulation of grid-based NeRF~\cite{dvgo,plenoxels,instant-ngp}.
In sum, our \ourshortname, like grid-based NeRF, supports volumetric rendering while maintaining the efficiency of 3DGS achieving $>\!\!100$ FPS for one-mega-pixels images.

Thanks to the fully explicit and volumetric property, we can directly incorporate some useful grid methods into our \ourshortname.
For instance, we can use sparse voxels to model SDF and use marching cubes to extract a mesh.
In addition, we can derive some gradient-descent-free methods to incorporate per-frame priors, \eg, visual hull from object masks and TSDF fusion from sensor depth.
We showcase the effectiveness of employing these direct grid manipulation methods to achieve instant object reconstruction in less than 0.1 seconds and smooth initial surface for indoor scenes.
Such a direct gradient-free approach for incorporating the per-frame priors is not straightforward with 3DGS-based methods.



% One efficiency advantage of 3DGS comparing to the grid-based NeRF comes from the rasterization as the rendering function.
% When a ray march to a point in volume ray casting, grid-based NeRF need a data structure, like dense n-d array~\cite{dvgo,tensorf}, dense pointer table~\cite{plenoxels}, or hash grid~\cite{instant-ngp}, to efficiently access to the target voxel of the query point.
% On the other hand, 3DGS do not have to maintain a data structure as it just need to sort the Gaussians for blending the Gaussians in front-to-back order to form pixel colors.
% This property gives 3DGS flexibility to adapt its Gaussians explicitly to different level-of-details of the scene.
% ....can also skip free space without needing to check a dense occupancy grid employed by grid-based NeRF.


% Different from the volume ray casting employed by NeRF-family, 3DGS uses rasterization as the rendering function which brings the rendering FPS to the next level (\textgreater 100 FPS).
% One efficiency advantage of using rasterization is that the data structure for scene representation can be flexible.
% When using the grid-based NeRF with volume ray casting, we need a data structure, like structural n-d array or hash-grid, for efficient arbitrary 3D points query.
% Even with the sparse grid in Plenoxels~\cite{plenoxels}, they still need to maintain a dense 3D grid for storing the pointer to the sparse voxels.
% Conversely in rasterization, the primitives (the Gaussians in 3DGS) can be stored non-structurally and we just need to sort them for rendering in front-to-back order.

% One big advantage on the efficiency aspect is that some computation can be shared among pixels like the evaluation of the view-dependent color and the geometric projection of a Gaussian primitive.


==> sec/legacy/2_related_work.tex <==
\section{Related work}
\label{sec:related_work}

We give a high-level background context in this section. Some closely related works are discussed in the later sections.

\paragraph{Neural radiance fields}

\paragraph{Gaussian Splatting}



\paragraph{Discussion with 3DGS~\cite{3dgs}.}
\chengs{Cheng: Park here temporary.}
The Octree layout makes it simple to ensure the following important properties for the scene function and the rendering function.
First, we can easily prevent voxels overlapping, which causes rendering-order ambiguity and one-to-many mapping as a volumetric function, by removing parent voxels after subdivision.
Second, we can ensure exact front-to-back voxel rendering order, which will be detailed in~\cref{ssec:rasterization}, without the popping artifact~\cite{stopthepop} in 3DGS~\cite{3dgs}.

\jchoe{@Cheng, I think the paragraph below looks wrong. Some method allocates sparse voxel to volume-of-interest, which is a fine-grained approach. So, for me, it will be better to mention that we are free from quering voxel by simply using the rasterization. That will be good enough in my opinion.}
\paragraph{Discussion with grid-based NeRFs~\cite{dvgo,plenoxels,tensorf,instant-ngp}.}
\chengs{Cheng: Park here temporary.}
The Octree layout is flexible to fit into different Level-of-Detail (LoD) by allocating finer voxels to complex region and removing voxels from the empty space.
Conversely, previous grid-based NeRFs allocate voxels uniformly for the entire 3D scene, \ie, they do not apply finer grid only for certain local region and using a finer grid imply the grid is finer everywhere in 3D.
For instance, the hash table for a resolution is shared by the entire 3D~\cite{instant-ngp}; the sparse grid in previous method~\cite{plenoxels} still need a 3D dense pointer grid for ray marching.
Further, grid-based NeRFs still need to maintain and query a dense occupancy grid to skip empty space while we just need to remove the empty voxels.

==> sec/legacy/3_our_renderer-origin.tex <==
\section{\ourfullname}
\label{sec:approach}

We introduce our \ourfullname (\ourshortname) in a bottom-up manner in this section.
First, we describe the most fundamental voxel units and their rendering given a pixel ray in \cref{ssec:scene_repr}.
We detail the layout structure design of these voxels to form the 3D scenes in \cref{ssec:scene_layout}, and the rendering algorithm to form 2D views in \cref{ssec:scene_rend}.

%
% Our scene representation
%
\subsection{Preliminary: voxel rendering}
\label{ssec:scene_repr}
\jchoe{TODO: make this subsection shorter. discussed by Cheng.}
We start by reviewing the common rendering formulation with some of our adaptation.
Sparse voxel representation~\cite{mink,spconv,plenoxels,instant-ngp} is widely used to compose 3D scenes with sparsely allocated voxels.
% Each voxel is parameterized as a feature vector $\voxmod \in \Real^d$ at a voxel location $\voxcen = [i, j, k] \in \Int^3$ where $d$ is the dimension of the feature and a voxel size is pre-defined as $\voxsiz \in \Real$.
Each voxel region is parameterized by a voxel center $\voxcen \in \Real^3$ and a voxel size $\voxsiz \in \Real$.
Based on this framework, we sub-divide the sparse voxel representations into (1) constant voxel field and (2) tri-linear voxel field as depicted in \cref{fig:voxel_field}.
% In convention, each voxel is parameterized as voxel location $\voxcen \in \Real^3$, and voxel size $\voxsiz \in \Real$.
% Our scene is consisting of a set of voxels sparsely allocated in 3D space. The region of a voxel is defined by it's voxel center $\voxcen \in \Real^3$, voxel size $\voxsiz \in \Real$.
% We implement the following two voxel field for the modal of interest, which are also depicted in \cref{fig:voxel_field}.
% \jchoe{@Cheng, Both types of voxel fields are not somthing new. So, I re-write the contents as it is. Please feel free to fix it as you like}



\paragraph{Constant voxel field.}
% Previously, sparse voxel representation is simply discretization of pointclouds~\cite{mink} based on the predefined voxel size~$\voxsiz$. Given a query point~$\mathbf{p} = [x, y, z] \in \Real^3$, sparse voxel is indexed by referring to a hash map. Then, we obtain a feature vector at a queried voxel~$\voxmod \in \Real^d$, such as color, location, or feature vector. If there is no voxel at the query, it returns a zero vector.
The simplest model is to treat the feature are constant inside a voxel modeled by $\voxmod \in \Real^d$ of each voxel where $d$ is the dimension of the feature. 
% we obtain a raw value of the queried voxels~$\voxmod \in \Real^d$, such as color, location, or feature vector.
% Given a sparse grid, the simplest sampling method is a Nearest interpolation. This technique assumes that the voxel features are constant insdie 


\paragraph{Tri-linear voxel field.}
% In a recent method~\cite{instant-ngp}, this method designs a hash grid that maps continuous coordinates to sparsely distributed voxels. Based on this pre-defined hash map, tri-linear interpolation is used to sample a feature vector at a query point $\mathbf{p}$ that is adjacent to the eight grid voxels (\ie, corners) $\voxmod \in \Real^{8\times d}$. Then, it linearly interpolates the query features from the 8-neighbors voxel features.
% Despite its merits, this algorithm does not re-compute the hash map depending on the target 3D scenes but pre-compute the occupancy map to avoid a hash collision problem~\cite{dong2023fast}. Accordingly, this method~\cite{instant-ngp} potentially can encounter the hash collision problem.
Another commonly used voxel model is tri-linear field by interpolating from the features attached to the eight grid points (\ie, corners) of a voxel $\voxmod \in \Real^{8\times d}$.
Note that we merge all the duplicated grid points from all the voxels to form a grid points feature pool $\gridmod \in \Real^{\nunq \times d}$, where $\nunq$ is the number of unique grid points.
This greatly reduces the number of parameters by parameters sharing between adjacent voxels and avoids the ambiguous one-to-many mapping as a volumetric function.


In the task of novel-view synthesis, the voxel modal of interest are geometry and view-dependent appearance.
Given a pixel ray $\ray$, we finally want to derive the voxel alpha value $\voxalp(\ray) \in \Realprob$ and voxel rgb intensity $\voxrgb(\ray) \in \Realnonneg^3$ as a function of rays.
Let $\rayo \in \Real^3$ be the origin and $\rayd \in \Real^3$ be the direction of the ray.
We first need to compute ray-aabb intersection to find the entrance $(\rayo + a \rayd)$ and exit $(\rayo + b \rayd)$ positions on the voxel surface if the ray hit the voxel.
We describe several instantiations with different pros and cons in the following.

\paragraph{Constant density.}
The simplest geometry model is using constant field to model the volume density with a trainable parameter $\voxgeo \in \Real^1$ attached to a voxel.
We use exponential-linear activation function to ensure non-negative density:
\begin{equation} \label{eq:explin}
    \explin(x) = \begin{cases}
        x & \text{if } x > 1.1\\
        \exp\left(\frac{x}{1.1} -1+\ln1.1\right)& \text{otherwise}
    \end{cases} ~,
\end{equation}
which is smoother than $\relu$ and more efficient to evaluate than $\softplus$.
We follow NeRF to use classical volume rendering equation~\cite{Kajiya,Max} to define the voxel alpha value for the ray:
\begin{equation}
    \voxalp(\ray) = 1 - \exp(-I) ~,
\end{equation}
where $I$ is the integrated volume density along the ray segment $[a, b]$.
For constant density, the integral is simply:
\begin{equation} \label{eq:integral_constant}
    I = \explin(\voxgeo) \cdot (b - a) \cdot \|\rayd\| ~,
\end{equation}
where $((b - a) \cdot \|\rayd\|)$ is the length of the ray segment.

\paragraph{Tri-linear density.}
Modeling voxel geometry by tri-linear voxel $\voxgeo \in \Real^{8\times 1}$ leads to better result quality while requires more computation.
A closed-form integral of tri-linear field is too complicated so we use quadrature with $\nsamp$ samples using mid-point rule:
\begin{equation} \label{eq:integral_trilinear}
    I = \frac{(b - a) \cdot \|\rayd\|}{\nsamp} \cdot \sum_i^{\nsamp} \explin(\interp(\voxgeo, \rayq_i))  ~,
\end{equation}
where $\rayq_i$ is the $i$-th sample under the normalized coordinate of the voxel.
We defer the detail equation of $\rayq_i$ in supplementary.

% \paragraph{Linear density.}
% \chengs{To be decided... in this mode, we derive a linear field so we can have closed-form integral... but need more discussions as the merit is not so clear.}

\paragraph{Signed distance.}
Modeling geometry as signed distance field is shown to be better for NeRF-based mesh reconstruction techniques~\cite{neus,volsdf}.
We also implement VolSDF~\cite{volsdf}'s formulation of using the Cumulative Distribution Function of the Laplacian distribution to map signed distance (SDF) to volume density.
Specifically, we use the following activation function to replace \cref{eq:explin} when modeling the scene with signed distance field instead of density field:
\begin{equation}
    \volsdf(x) = 0.5 \alpha (1 - \sgn(x) + \sgn(x)\exp(-\beta |x|) ~,
\end{equation}
where $\sgn$ is the sign of the variables, $\alpha$ is the maximum density, and $\beta$ controls the surface sharpness.
Both $\alpha$ and $\beta$ can be trainable or heuristically scheduled.

\paragraph{Spherical harmonics.}
Finally, we use spherical harmonic (SH) with $\nshd$ degree to model the view-dependent appearance of each voxel.
In case of constant voxel field, each voxel has $\voxshs \in \Real^{3(\nshd+1)^2}$ trainable parameters with the final voxel color for the ray be:
\begin{equation}
    \voxrgb(\ray) = \max(0, \sheval(\voxshs, \rayd)) ~,
\end{equation}
where $\sheval$ map SH coefficients and ray direction to rgb intensity.
For trilinear voxel field, each voxel is attached with $\voxshs \in \Real^{8\times 3(\nshd+1)^2}$ grid points SH coefficients.
For efficiency, we use a pre-activation scheme (\ie, turning into rgb field first) and only sample one point:
\begin{equation}
    \voxrgb(\ray) = \interp(\sheval(\voxshs, \rayd), \rayq_{\mathrm{mid}}) ~,
\end{equation}
where $\rayq_{\mathrm{mid}}$ is at the middle of the ray segment $[a,b]$.
We follow prior works~\cite{3dgs,plenoxels} to only clamp negative to zero.


%
% Our scene structure
%
\subsection{Octree grid layout}
\label{ssec:scene_layout}
We design the layout of our sparse voxels to follow Octree space partition rule.
An 2D example is illustrated in \cref{fig:order_example}.
Despite sacrificing the freedom to optimize the center position and size of each voxel, we can still adapt the sparse voxels to the different scenes level-of-detail (LoD) by subdividing voxels during optimization.
Note that we do not maintain the Octree data structure, \ie the pointer to parent and children nodes, for rendering.
Our rasterizer (\cref{ssec:scene_rend}) sorts the voxel for each ray to iterate from front-to-back order so we do not need the Octree data structure for the rays to traverse and locate the voxels to render.
Thanks to the flexibility provided by the rasterizer, we just store each individual voxels in arbitrary order.

\paragraph{Discussion with 3DGS~\cite{3dgs}.}
The Octree layout makes it simple to ensure the following important properties for the scene function and the rendering function.
First, we can easily prevent voxels overlapping, which causes rendering-order ambiguity and one-to-many mapping as a volumetric function, by removing parent voxels after subdivision.
Second, we can ensure exact front-to-back voxel rendering order, which will be detailed in \cref{ssec:scene_rend}, without the popping artifact~\cite{stopthepop} in 3DGS~\cite{3dgs}.

\paragraph{Discussion with grid-based NeRFs~\cite{dvgo,plenoxels,tensorf,instant-ngp}.}
The Octree grid layout is more flexible to fit into different LoD by allocating finer voxels to complex region and removing voxels from the empty space.
Conversely, previous grid-based NeRFs allocate voxels uniformly for the entire 3D scene, \ie, they do not apply finer grid only for certain local region and using a finer grid imply the grid is finer everywhere in 3D.
For instance, the hash table for a resolution is shared by the entire 3D~\cite{instant-ngp}; the sparse grid in previous method~\cite{plenoxels} still need a 3D dense pointer grid for ray marching.
Further, grid-based NeRFs still need to maintain and query a dense occupancy grid to skip empty space while we just need to remove the empty voxels.


%
% Our rasterization algorithm
%
\subsection{Rasterization algorithm}
\label{ssec:scene_rend}



One remaining challenge is about the rendering order.
Naively sorting the voxels by center or nearest corner position can result in incorrect order as depicted in \cref{fig:incorrect_order}.
Such an incorrect ordering issue also exhibits in 3DGS which causes multi-view inconsistency and popping artifact~\cite{stopthepop}.
Thanks to the Octree grid layout (\cref{ssec:scene_layout}), we can use a multi-levels Z-order encoding to ensure correct rendering order.
We use a 2D example in \cref{fig:cam_quad_and_order} for explanation.
The camera origin partition the 2D space into four camera quadrants.
We can then build an ordering table for each camera quadrant to decide the rendering order of any four sibling voxels, which ensures correct rendering order for all the rays casting into the camera quadrant.
Finally, extending the encoding to multilevel yields correct ordering for the sparse voxels, where an example is depicted in \cref{fig:order_example}.
We generalize the order encoding to 3D with eight camera quadrants and ordering tables.
In case a voxel touch multiple camera quadrants, we duplicates the voxels with different order encodings of the quadrants.
% CUDA-level implementation details are provided in the supplementary.

To achieve real-time rendering, we build our tile-based sparse voxels rasterizer as a differentiable Pytorch CUDA extention following the efficient implementation from 3DGS~\cite{3dgs}.
The rasterizer gathers a sequence of voxel indices sorted by the order encoding for each tile (\ie, image patch).
Let $k$ be the list of $\nlst$ indices assigned to the tile where a pixel ray $\ray$ belonging to.
We finally can perform alpha composition to render the pixel color:
\begin{subequations} \label{eq:alpha_blend}
\begin{align}
    \pixrgb(\ray) &= \sum\nolimits_{i=1}^{\nlst} T_i \cdot \alpha_i \cdot \voxrgb^{(k_i)}(\ray) ~, \\
    T_i &= \prod\nolimits_{j=1}^{i-1} \left(1 - \alpha_j\right) ~, \\
    \alpha_i &= \voxalp^{(k_i)}(\ray) \cdot \mathrm{hit}(\ray,\vox^{(k_i)}) ~,
\end{align}
\end{subequations}
where $\mathrm{hit}$ indicate if a (duplicated) voxel is both intersected with the ray and align with the quadrant of the ray in case an image tile covering multiple camera quadrant.
We do early ray stopping after the transmittance below a threshold $T_i{<}\hypertstop$.
More low-level implementation of the rasterizer are detailed in the supplementary.

\paragraph{Anti-aliasing.}
To mitigate aliasing artifact, we use super-sampling strategy by rendering in $\hyperss$ times higher resolution and then downsampling the rendered views to the target resolution.

\paragraph{Global pre-sorting.}
We apply per-frame sorting similar to 3DGS.
One characteristic of our order encoding indicating that there are only eight possible sorting results globally for all the camera positions, which means that we can actually pre-sort the voxels once as pre-processing and waive the per-frame sorting in the rendering pipeline.
However, we do not find any efficiency advantage in our experiments by the global pre-sorting.
More future analysis is needed for this feature and we use the simpler per-frame sorting now.


==> sec/legacy/4_1.tex <==
%
% Sparse Grid Layout
%
\subsection{Sparse grid layout}
\label{ssec:sparse_grid_layout}
\jchoe{
Our \ourshortname constructs 3D scenes in sparse voxel representation. Each sparse voxel~$\vox$ is parameterized as a voxel center $\voxcen \in \Real^3$ and a voxel size $\voxsiz \in \Real$. Each voxel has 8 eight grid points (\ie, corners) that stores feature vectors~$\voxmod \in \Real^{8\times d}$. 
Note that we merge all the duplicated grid points from all voxels to form a unified grid points feature pool $\gridmod \in \Real^{\nunq \times d}$, where $\nunq$ is the number of unique grid points. This greatly reduces the number of parameters by parameters sharing between adjacent voxels and avoids the ambiguous one-to-many mapping as a volumetric function.

The layout of our sparse voxels follows Octree space partition rule.
An 2D example is illustrated in~\cref{fig:order_example}.
Despite sacrificing the freedom to optimize the center position and size of each voxel, we can still adapt the sparse voxels to the different scenes level-of-detail (LoD) by subdividing voxels during optimization.
Note that we do not maintain the Octree data structure, \ie the pointer to parent and children nodes, for rendering.
Our rasterizer (\cref{ssec:rasterization}) sorts the voxel for each ray to iterate from front-to-back order so we do not need the Octree data structure for the rays to traverse and locate the voxels to render.
Thanks to the flexibility provided by the rasterizer, we just store each individual voxels in arbitrary order.

\paragraph{Discussion with 3DGS~\cite{3dgs}.}
The Octree layout makes it simple to ensure the following important properties for the scene function and the rendering function.
First, we can easily prevent voxels overlapping, which causes rendering-order ambiguity and one-to-many mapping as a volumetric function, by removing parent voxels after subdivision.
Second, we can ensure exact front-to-back voxel rendering order, which will be detailed in~\cref{ssec:rasterization}, without the popping artifact~\cite{stopthepop} in 3DGS~\cite{3dgs}.

\paragraph{Discussion with grid-based NeRFs~\cite{dvgo,plenoxels,tensorf,instant-ngp}.}
The Octree grid layout is more flexible to fit into different LoD by allocating finer voxels to complex region and removing voxels from the empty space.
Conversely, previous grid-based NeRFs allocate voxels uniformly for the entire 3D scene, \ie, they do not apply finer grid only for certain local region and using a finer grid imply the grid is finer everywhere in 3D.
For instance, the hash table for a resolution is shared by the entire 3D~\cite{instant-ngp}; the sparse grid in previous method~\cite{plenoxels} still need a 3D dense pointer grid for ray marching.
Further, grid-based NeRFs still need to maintain and query a dense occupancy grid to skip empty space while we just need to remove the empty voxels.


%
% Our rasterization algorithm
%
\subsection{Rasterization algorithm}
\label{ssec:rasterization}
For the accurate rasterization process, rendering order is an important issue. 
Naively sorting the voxels by center or nearest corner position can result in incorrect order as depicted in~\cref{fig:incorrect_order}. Such an incorrect ordering issue also exhibits in 3DGS which causes multi-view inconsistency and popping artifact~\cite{stopthepop}. 
Thanks to the Octree grid layout (\cref{ssec:sparse_grid_layout}), we adopt a multi-levels Z-order encoding to ensure correct rendering order. We use a 2D example in~\cref{fig:cam_quad_and_order} for explanation. The camera origin partition the 2D space into four camera quadrants. We can then build an ordering table for each camera quadrant to decide the rendering order of any four sibling voxels, which ensures correct rendering order for all the rays casting into the camera quadrant. Finally, extending the encoding to multi-level yields correct ordering for the sparse voxels, where an example is depicted in~\cref{fig:order_example}. We generalize the order encoding to 3D with eight camera quadrants and ordering tables. In case a voxel touch multiple camera quadrants, we duplicates the voxels with different order encodings of the quadrants. 
% CUDA-level implementation details are provided in the supplementary.

To achieve real-time rendering, we build our tile-based sparse voxels rasterizer as a differentiable Pytorch CUDA extention following the efficient implementation from 3DGS~\cite{3dgs}.
The rasterizer gathers a sequence of voxel indices sorted by the order encoding for each tile (\ie, image patch).
Let $k$ be the list of $\nlst$ indices assigned to the tile where a pixel ray $\ray$ belonging to.
We finally can perform alpha composition to render the pixel color:
\begin{subequations} \label{eq:alpha_blend}
\begin{align}
    \pixrgb(\ray) &= \sum\nolimits_{i=1}^{\nlst} T_i \cdot \alpha_i \cdot \voxrgb^{(k_i)}(\ray) ~, \\
    T_i &= \prod\nolimits_{j=1}^{i-1} \left(1 - \alpha_j\right) ~, \\
    \alpha_i &= \voxalp^{(k_i)}(\ray) \cdot \mathrm{hit}(\ray,\vox^{(k_i)}) ~,
\end{align}
\end{subequations}
where $\mathrm{hit}(\cdot)$ indicate if a (duplicated) voxel is both intersected with the ray and align with the quadrant of the ray in case an image tile covering multiple camera quadrant.
We do early ray stopping after the transmittance below a threshold $T_i{<}\hypertstop$.
More low-level implementation of the rasterizer are detailed in the supplementary.

\paragraph{Anti-aliasing.}
To mitigate aliasing artifact, we use super-sampling strategy by rendering in $\hyperss$ times higher resolution and then downsampling the rendered views to the target resolution.

\paragraph{Global pre-sorting.}
We apply per-frame sorting similar to 3DGS.
One characteristic of our order encoding indicating that there are only eight possible sorting results globally for all the camera positions, which means that we can actually pre-sort the voxels once as pre-processing and waive the per-frame sorting in the rendering pipeline.
However, we do not find any efficiency advantage in our experiments by the global pre-sorting.
More future analysis is needed for this feature and we use the simpler per-frame sorting now.

\input{fig/order}


%
% Our differential rendering to predict pixel colors
%
\subsection{Differential rendering}
\label{ssec:differential_rendering}

In the task of novel-view synthesis, the voxel modal of interest are geometry and view-dependent appearance.
Given a pixel ray $\ray$, we finally want to derive the voxel alpha value $\voxalp(\ray) \in \Realprob$ and voxel rgb intensity $\voxrgb(\ray) \in \Realnonneg^3$ as a function of rays.
Let $\rayo \in \Real^3$ be the origin and $\rayd \in \Real^3$ be the direction of the ray.
We first need to compute ray-aabb intersection to find the entrance $(\rayo + a \rayd)$ and exit $(\rayo + b \rayd)$ positions on the voxel surface if the ray hit the voxel. Based on this framework, we design voxels for geometry and view-dependent appearance.

In our geometry voxels, we use exponential-linear activation function to ensure non-negative density:
\begin{equation} \label{eq:explin}
    \explin(x) = \begin{cases}
        x & \text{if } x > 1.1\\
        \exp\left(\frac{x}{1.1} -1+\ln1.1\right)& \text{otherwise}
    \end{cases} ~,
\end{equation}
which is smoother than $\relu$ and more efficient to evaluate than $\softplus$.
We follow NeRF to use classical volume rendering equation~\cite{Kajiya,Max} to define the voxel alpha value for the ray:
\begin{equation}
    \voxalp(\ray) = 1 - \exp(-I) ~,
\end{equation}
where $I$ is the integrated volume density along the ray segment $[a, b]$. 
A closed-form integral of tri-linear field is too complicated so we use quadrature with $\nsamp$ samples using mid-point rule:
\begin{equation} \label{eq:integral_trilinear}
    I = \frac{(b - a) \cdot \|\rayd\|}{\nsamp} \cdot \sum_i^{\nsamp} \explin(\interp(\voxgeo, \rayq_i))  ~,
\end{equation}
where $\rayq_i$ is the $i$-th sample under the normalized coordinate of the voxel.
We defer the detail equation of $\rayq_i$ in supplementary.

For view-dependent appearance, we use spherical harmonic (SH) with $\nshd$ degree to model the view-dependent appearance of each voxel.
In case of constant voxel field, each voxel has $\voxshs \in \Real^{3(\nshd+1)^2}$ trainable parameters with the final voxel color for the ray be:
\begin{equation}
    \voxrgb(\ray) = \max(0, \sheval(\voxshs, \rayd)) ~,
\end{equation}
where $\sheval$ map SH coefficients and ray direction to rgb intensity.
For trilinear voxel field, each voxel is attached with $\voxshs \in \Real^{8\times 3(\nshd+1)^2}$ grid points SH coefficients.
For efficiency, we use a pre-activation scheme (\ie, turning into rgb field first) and only sample one point:
\begin{equation}
    \voxrgb(\ray) = \interp(\sheval(\voxshs, \rayd), \rayq_{\mathrm{mid}}) ~,
\end{equation}
where $\rayq_{\mathrm{mid}}$ is at the middle of the ray segment $[a,b]$.
We follow prior works~\cite{3dgs,plenoxels} to only clamp negative to zero.






==> sec/legacy/5_5_demo.tex <==
\subsection{More results}
\label{ssec:demo}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \subsection{Visual hull carving}
% \label{ssec:exp_visual_hull}

% We demonstrate the results by incorporating visual hull into our model in \cref{fig:exp_visual_hull}.
% Thanks to the sparsity and fully explicit property of our representation, we can start our method from a dense grid and easily remove those voxels carved by the provided object masks.
% By unproject the pixel colors to the carved sparse voxels, we can achieve a reasonable novel-view synthesis result without any training.
% The overall process take less than $0.1$ seconds.
% Starting from the carved voxels, we can further refine our model by 1K iterations (with less than $10$ seconds) and achieve high-quality rendering.
% The shown shape-from-silhouette ability of our method can facilitate fast and high-quality object reconstruction pipeline.

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \subsection{TSDF fusion}
% \label{ssec:exp_tsdf_fusion}

% Our sparse voxel representation can also be employed to perform TSDF fusion as demonstrated in \cref{fig:exp_tsdf_fusion}.
% Without any training, we can achieve a smooth surface as shown by the rendered depth and normal maps from our representation.
% Different from the classical Volume fusion techniques employed for mesh extraction, our \ourshortname can further be refined as a volumetric 3D model for better novel-view synthesis quality and, potentially, finer geometry details.

==> supp_material/fig/qual_more_nvs.tex <==
\begin{figure*}[h]
    \centering
    \includegraphics[width=\linewidth]{supp_material/img/qual_more_nvs.pdf}
    % \vspace{-2em}
    \caption{
    {\bf Qualitative novel-view rendering results on-par with 3DGS.}
    }
    \label{fig:qual_more_nvs}
\end{figure*}

==> tab/technical_comparison.tex <==
\begin{table*}[!t]
    \centering
    \resizebox{1\linewidth}{!}{
        \begin{tabular}{ccccccc}
            \toprule
            Methods                        & Data structure & Scene representation & Rasterization & Rendering speed (FPS) & Quality (PSNR) & Memory (MB) \\ 
            \midrule
            % Mink Engine & Sparse hash      & Voxel                &               & -                     &                \\
            % fVDB
            NeRF~\cite{nerf}               & & &               & &                & \\
            Instant-NGP~\cite{instant-ngp} & Dense hash     & Voxel + MLP          & & $\sim$10              & &\\
            Plenoxel~\cite{plenoxels}      & Octree         & Voxel                &               & $\sim$10              &                & \\
            \midrule
            3DGS~\cite{3dgs}               & Array          & Gaussian             & $\checkmark$  & 132                   &                & \\
            3DGRT~\cite{3dgrt}             & Array          & Gaussian             &               & 40                    &                & \\
            \midrule
            SVR (Ours)                     & Array          & Voxel                & $\checkmark$  & 134                   &                & \\
            \bottomrule
        \end{tabular}
    }
    \caption{Technical comparisons.}
    \label{tab:technical_comparison}
\end{table*}


